SEVERE++: Evaluating Benchmark Sensitivity in Generalization of Video Representation Learning

Continued advances in self-supervised learning have led to significant progress in video representation learning, offering a scalable alternative to supervised approaches by removing the need for manual annotations. Despite strong performance on standard action recognition benchmarks, video self-supervised learning methods are largely evaluated under narrow protocols, typically pretraining on Kinetics-400 and fine-tuning on similar datasets, limiting our understanding of their generalization in real world scenarios. In this work, we present a comprehensive evaluation of modern video self-supervised models, focusing on generalization across four key downstream factors: domain shift, sample efficiency, action granularity, and task diversity. Building on our prior work analyzing benchmark sensitivity in CNN-based contrastive learning, we extend the study to cover state-of-the-art transformer-based video-only and video-text models. Specifically, we benchmark 12 transformer-based methods (7 video-only, 5 video-text) and compare them to 10 CNN-based methods, totaling over 1100 experiments across 8 datasets and 7 downstream tasks. Our analysis shows that, despite architectural advances, transformer-based models remain sensitive to downstream conditions. No method generalizes consistently across all factors, video-only transformers perform better under domain shifts, CNNs outperform for fine-grained tasks, and video-text models often underperform despite large scale pretraining. We also find that recent transformer models do not consistently outperform earlier approaches. Our findings provide a detailed view of the strengths and limitations of current video SSL methods and offer a unified benchmark for evaluating generalization in video representation learning.

==> sections/conclusion.tex <==
\section{Conclusion} 
In this work, we thoroughly evaluated the generalization of a set video self-supervised learning models beyond standard downstream benchmarks. We identify four sensitivity factors in the downstream \ie domain, samples, semantic similarity and the nature of task, that impact the generalization of video self-supervised pre-training. Our comprehensive set of experiments reveals that current benchmarks in video self-supervised learning are not a good indicator of generalization along the said sensitivity factors. Further, we found that self-supervised methods significantly lag behind supervised pre-training especially when domain shift is high, the amount of downstream samples are low, for fine-grained action classification with high similarities and when there is both domain and task shift. Finally, we propose a subset of our experiments as an alternative benchmark to evaluate future works in video self-supervised learning for generalization beyond current standard evaluation and close the gap with supervised training.

%As well as being more generalizable to different domains, supervised pre-training is much more generalizable when there is a limited amount of training data in the downstream task. There are currently no self-supervised approaches successful when both the amount of downstream training data is reduce and when there is a change in domain.% with a change in domain and size of the downstream dataset.

% Summarizing these results, we see that compared to supervised pre-training, self-supervised pre-training often struggles to generalize to different domains especially in a low-data regime. There is currently no approach successful in all settings, with % supervised pre-training dominates self-supervised pre-training  for most transfer settings especially in low-data regime. While the best 
% self-supervised methods rank differently with change in domain and size of the downstream dataset.

%This is likely due to the large number of temporal augmentations it uses  encourages robustness to 
 %which helps the generalization ability when finetuning data is limited. %However, invariance to time reversal seems to harm its performance with increasing training data for SS-v2 and GYM-99  which contains action with temporal direction labels.
%To-do add short summary for whole domain shift section

%This is likely because the CtP pre-text task is very different from classification, thus more finetuning is needed to make use of the features it learns. %For example, CtP  ranks much higher  with increasing finetuning  data for UCF, GYM and SS-v2. %
%

%It also suggests that the tracking based pretext task in CtP may be more effective than contrastive tasks for distinguishing subtle differences in motion. 
%This suggests that the additional temporal tasks video self-supervised methods introduce can harm performance on more semantically similar subsets. For instance, in GDT the invariance to temporal reversal harms the ability to distinguish between backward and forward movements which is needed in UB-S1. %is worse than MoCo on finer-grained Gym-99 subsets suggesting that  invariance to frame dropout in VideMoCo can harm the performance on finer granularities with highly similar actions. 
%For GDT it is likely that the temporal reversal invariance harms the ability to distinguishing between backward or forward movements in the uneven bars circles subset (UB-S1).
%we believe this is due to the very intense motions in actions from this event. % and  high similarity among actions, e.g. \textit{salto with 2.0 twist off} and \textit{salto with 2.5 twist off}. 
%Generally, the ranking of methods is similar in Gym-288 and Gym-99, indicating that the domain and granularity are more important factors in deciding the suitability of the self-supervised method.

%One explanation is that it contrasts between different parts of the same video clip which may result in better learning of long-term features than other methods. 

%\subsection{Does self-supervised pre-training learn same features as the supervised pre-training?}
%\hd{TO DO}

==> sections/related_work.tex <==
%\section{Related Works}
%Most video self-supervised learning methods  \cite{rotate1-jing2019selfsupervised, shuffle1-fernando2017self} use unlabeled Kinetics-400~\cite{Kinetics-400-arxiv} for pre-training and then measure performance by finetuning and testing on two action recognition datasets: UCF-101~\cite{UCF-101-arxiv} and HMDB-51~\cite{HMDB-51-ICCV}. Some works~\cite{gdt-patrick2020multimodal, dave2021tclr, pretext-contrast-DBLP:journals/corr/abs-2010-15464, ctp-wang2021unsupervised, rspnet-chen2020RSPNet, selavi-asano2020labelling} also report performance on video retrieval for UCF-101 and HMDB-51 and 
%several recent works~\cite{qian2021spatiotemporal,yang2020video,recasens2021broaden} compare linear-evaluation performance on Kinetics-400. While these benchmarks have demonstrated the effectiveness of self-supervised learning for video, they do not indicate the generalizability of such methods as these datasets are all similar in appearance and the type of actions they contain. 
% Some methods have started to report finetuning performance on additional datasets like
% Something-Something-v2~\cite{SS-v2-arxiv} in~\cite{ctp-wang2021unsupervised,rspnet-chen2020RSPNet,large-scale-feichtenhofer2021large}, Diving-48~\cite{diving} in~\cite{dave2021tclr,wang2021removing}, AVA~\cite{AVA-Gu_2018_CVPR} in~\cite{xiao2021modist,yang2020video,large-scale-feichtenhofer2021large}, EPIC-Kitchens~\cite{EPIC-100-arxiv} in~\cite{yang2020video}.  %Others~\cite{qian2021spatiotemporal,yang2020vthcl,recasens2021broaden} follow  the trend in image self-supervised learning to report linear-evaluation performance on Kinetics-400. Hence, there is no  proper benchmark  that can be used to thoroughly evaluate video self-supervised methods. 
% However, such evaluations are insufficient to understand the generalization of video self-supervised methods since they only add a single additional dataset, often without comparison to prior methods. 
% In this work, we investigate the sensitivity of standard video self-supervised evaluation to four different downstream factors by conducting a large-scale study of video self-supervised models. From this we propose a benchmark for future video self-supervsied works can use to measure generalizability.
 

%\subsection{Evaluations protocols in self-supervised learning.} 



%\cite{large-scale-feichtenhofer2021large} extended 4 popular  image-based methods SimCLR \cite{simclr-pmlr-v119-chen20j}, MoCo \cite{moco}, SWAV~\cite{swav} and BYOL~\cite{byol} for video data. They analyse these methods  for various design choices  such as network architectures, pre-training datasets, temporal persistence ,data augmentations and downstream performance.
%In contrast to image-based evaluations, video presents a challenge since it introduces multiple axes of variations. 
%Unlike \cite{large-scale-feichtenhofer2021large}, we fix the pre-training setup and focus on generalizability across various factors driving the downstream evaluation.



%\medskip
%\noindent\textbf{Analysis of Self-Supervised Representations.} 
%Several works have performed similar benchmarking studies in images~\cite{when_contrast_work,trasnferability,contrasting_contrastive,edinburgh-ericsson2021well, goyal2019scaling, yang2020transfer, kolesnikov2019revisiting, zhai2019large, asano2019critical, newell2020useful, sariyildiz2021concept, van2021benchmarking, ericsson2021self} with the goal of examining generalization beyond ImageNet \cite{deng2009imagenet}. %For example, Cole~\etal\cite{when_contrast_work}
%%analyse how the pre-training dataset impacts performance of SimCLR on different downstream benchmarks and conclude that contrastive learning lags behind supervised pre-training for various downstream settings like low-data regime and fine-grained classification. Similarly, Kotar~\etal\cite{contrasting_contrastive} study 20 different downstream tasks and demonstrate lack of any strong correlation between ImageNet performance and out-of-domain tasks for contrastive learning methods. Ericsson~\etal\cite{edinburgh-ericsson2021well} keep the pre-training fixed and analyse the generalization of image self-supervised models to many-shot recognition, few-shot recognition, object detection and dense prediction to demonstrate that ImageNet performance is well correlated with many-shot recognition and less correlated to other downstream tasks. 
%However, video self-supervised methods are much distinct from image-based methods as video requires temporal \cs{and often multimodal} understanding in addition to spatial understanding. Thus the conclusions for image-based studies do not naturally transfer to videos and an independent study about generalization for videos is needed. Taking inspirations from the image-based studies, we aim to fill this gap in the current literature %However, no such study exists for video data, leaving a gap in analysis of current video self-supervised models. Our study aims to fill this gap 
%with a large-scale evaluation to investigate the generalization of current video self-supervised methods across a variety of downstream settings.
